Mixed--frequency quantile regressions to forecast Value--at--Risk and Expected Shortfall

Although quantile regression to calculate risk measures has been widely established in the financial literature, when considering data observed at mixed--frequency, an extension is needed. In this paper, a model is suggested built on a mixed--frequency quantile regression to directly estimate the Value--at--Risk (VaR) and the Expected Shortfall (ES) measures. In particular, the low--frequency component incorporates information coming from variables observed at, typically, monthly or lower frequencies, while the high--frequency component can include a variety of daily variables, like market indices or realized volatility measures. The conditions for the weak stationarity of the daily return process are derived and the finite sample properties are investigated in an extensive Monte Carlo exercise. The validity of the proposed model is then explored through a real data application using two energy commodities, namely, Crude Oil and Gasoline futures. Results show that our model outperforms other competing specifications, on the basis of some popular VaR and ES backtesting test procedures.

==> tables/backtesting_dow_jones.tex <==
\begin{table}[ht]
	\centering
		\caption{Dow Jones backtesting results}
		\vspace{-0.2cm}
	\label{tab:backtesting_dow_jones}
	\begin{adjustbox}{max width=0.8\textwidth}
	\begin{threeparttable}
\begin{tabular}{l  c ......}
\toprule
 &     \mc{LF var.} &          \mc{Mean} &         \mc{SD} &      \mc{AE} &     \mc{LR$_{uc}$} &       \mc{LR$_{cc}$} & \mc{DQ}\\
\midrule
 \cellcolor{gray!50}MF--Q--ARCH--X & $\Delta IP_t$ & -1.071 & 0.589 & 0.898 & 0.460 & 0.575 & 0.724 \\ 
 \cellcolor{gray!50}MF--Q--ARCH--X & $\Delta HS_t$ & -1.105 & 0.565 & 0.835 & 0.229 & 0.469 & 0.697  \\ 
 \cellcolor{gray!50}MF--Q--ARCH--X & $NAI_t$ & -1.097 & 0.583 & 0.856 & 0.295 & 0.568 & 0.801 \\ 
  \cellcolor{gray!50}MF--Q--ARCH & $\Delta IP_t$ & -1.065 & 0.481 & 0.981 & 0.894 & 0.259 & 0.528 \\ 
\cellcolor{gray!50}MF--Q--ARCH & $\Delta HS_t$ & -1.113 & 0.462 & 0.793 & 0.128 & 0.167 & 0.623 \\ 
 \cellcolor{gray!50}MF--Q--ARCH & $NAI_t$ & -1.089 & 0.476 & 0.919 & 0.558 & 0.144 & 0.545 \\ 
 \cellcolor{gray!50}Q--ARCH &  & -1.081 & 0.475 & 0.877 & 0.372 & 0.478 & 0.644 \\ 
  \cellcolor{gray!50}SAV &  & -0.980 & 0.456 & 1.044 & 0.757 & 0.356 & 0.835\\ 
   \cellcolor{gray!50}AS &  & -0.958 & 0.456 & 1.023 & 0.871 & 0.938 & 0.996 \\ 
  IG &  & -1.215 & 0.416 & 0.793 & 0.128 & 0.018 & 0.003  \\  
 GARCH &  & -1.185 & 0.407 & 0.814 & 0.173 & 0.028 & 0.006  \\ 
  GARCH--t &  & -1.152 & 0.416 & 0.877 & 0.372 & 0.023 & 0.010  \\ 
   \cellcolor{gray!50}GJR &  & -1.210 & 0.472 & 0.772 & 0.093 & 0.118 & 0.392  \\ 
   \cellcolor{gray!50}GJR--t &  & -1.181 & 0.500 & 0.835 & 0.229 & 0.302 & 0.598\\ 
 RiskMetrics &  & -1.206 & 0.465 & 0.772 & 0.093 & 0.011 & 0.003  \\ 
GARCH--MIDAS & $\Delta IP_t$ & -1.232 & 0.509 & 0.772 & 0.093 & 0.011 & 0.001 \\ 
 GARCH--MIDAS & $\Delta HS_t$ & -1.219 & 0.471 & 0.772 & 0.093 & 0.118 & 0.049 \\ 
 GARCH--MIDAS & $NAI_t$ & -1.220 & 0.502 & 0.856 & 0.295 & 0.003 & 0.000 \\ 

\bottomrule
 \end{tabular}
	\begin{tablenotes}[flushleft]
   \setlength\labelsep{0pt}
   \linespread{1.25}
\item  \textbf{Notes}:  The table reports the backtesting results for the models in the first column, for the out-of-sample period, which starts on May 2, 2016 and ends on February 28, 2020 (958 days). The models with the \virg{--X} label include the realized volatility (see Eq. \eqref{eq:larch_midas_x}). Column \virg{LF var.} reports the low--frequency variables.  Columns Mean and SD are the sample averages and standard deviations for the VaR measures. Column {AE} denotes the Actual over Expected exceedance ratio. Columns LR$_{uc}$ and LR$_{cc}$, report the p-values of the Unconditional and Conditional coverage tests. Finally, column DQ represents the p-value of the Dynamic Quantile test. Shades of gray denote that the model passes the LR$_{uc}$, LR$_{cc}$ and DQ tests at significance level $\alpha=0.05$.
\end{tablenotes}
\end{threeparttable}
	\end{adjustbox}
\end{table}












==> tables/backtesting_nasdaq.tex <==
\begin{table}[h]
	\centering
		\caption{NASDAQ backtesting results}
		\vspace{-0.2cm}
	\label{tab:backtesting_nasdaq}
	\begin{adjustbox}{max width=0.8\textwidth}
	\begin{threeparttable}
\begin{tabular}{l  c ......}
\toprule
 &     \mc{LF var.} &          \mc{Mean} &         \mc{SD} &      \mc{AE} &     \mc{LR$_{uc}$} &       \mc{LR$_{cc}$} & \mc{DQ}\\
\midrule
 \cellcolor{gray!50}MF--Q--ARCH--X & $\Delta IP_t$ & -1.305 & 0.593 & 1.001 & 0.994 & 0.927 & 0.971\\ 
   \cellcolor{gray!50}MF--Q--ARCH--X & $\Delta HS_t$ & -1.316 & 0.580 & 1.084 & 0.554 & 0.834 & 0.963 \\ 
 \cellcolor{gray!50}MF--Q--ARCH--X & $NAI_t$ & -1.302 & 0.590 & 1.189 & 0.192 & 0.416 & 0.821  \\ 
  \cellcolor{gray!50}MF--Q--ARCH & $\Delta IP_t$ & -1.313 & 0.461 & 1.189 & 0.192 & 0.403 & 0.260  \\ 
 \cellcolor{gray!50}MF--Q--ARCH & $\Delta HS_t$ & -1.343 & 0.454 & 1.084 & 0.554 & 0.834 & 0.185 \\ 
  \cellcolor{gray!50}MF--Q--ARCH & $NAI_t$ & -1.370 & 0.460 & 1.043 & 0.763 & 0.877 & 0.185 \\ 
\cellcolor{gray!50}Q--ARCH &  & -1.331 & 0.470 & 1.105 & 0.462 & 0.762 & 0.167 \\ 
SAV &  & -1.093 & 0.463 & 1.522 & 0.001 & 0.002 & 0.000  \\ 
AS &  & -1.076 & 0.510 & 1.502 & 0.001 & 0.003 & 0.023 \\ 
  \cellcolor{gray!50}IG &  & -1.405 & 0.343 & 0.938 & 0.659 & 0.904 & 0.117  \\
  \cellcolor{gray!50}GARCH &  & -1.307 & 0.360 & 1.084 & 0.554 & 0.724 & 0.210 \\ 
 GARCH--t &  & -1.264 & 0.366 & 1.189 & 0.192 & 0.416 & 0.018 \\ 
 \cellcolor{gray!50}GJR &  & -1.308 & 0.411 & 1.105 & 0.462 & 0.634 & 0.311 \\ 
\cellcolor{gray!50}GJR--t &  & -1.271 & 0.421 & 1.210 & 0.149 & 0.337 & 0.267  \\ 
  \cellcolor{gray!50}RiskMetrics &  & -1.355 & 0.446 & 1.022 & 0.877 & 0.930 & 0.133 \\ 
  \cellcolor{gray!50}GARCH--MIDAS & $\Delta IP_t$ & -1.321 & 0.372 & 1.022 & 0.877 & 0.930 & 0.275 \\ 
 \cellcolor{gray!50}GARCH--MIDAS & $\Delta HS_t$ & -1.335 & 0.365 & 1.043 & 0.763 & 0.877 & 0.137 \\ 
\cellcolor{gray!50}GARCH--MIDAS & $NAI_t$ & -1.294 & 0.386 & 1.168 & 0.245 & 0.369 & 0.003 \\ 
  
\bottomrule
 \end{tabular}
	\begin{tablenotes}[flushleft]
   \setlength\labelsep{0pt}
   \linespread{1.25}
\item  \textbf{Notes}:  The table reports the backtesting results for the models in the first column, for the out-of-sample period, which starts on May 2, 2016 and ends on February 28, 2020 (959 days). The models with the \virg{--X} label include the realized volatility (see Eq. \eqref{eq:larch_midas_x}). Column \virg{LF var.} reports the low--frequency variables. Columns Mean and SD are the sample averages and standard deviations for the VaR measures. Column {AE} denotes the Actual over Expected exceedance ratio. Columns LR$_{uc}$ and LR$_{cc}$, report the p-values of the Unconditional and Conditional coverage tests. Finally, column DQ represents the p-value of the Dynamic Quantile test. Shades of gray denote that the model passes the LR$_{uc}$, LR$_{cc}$ and DQ tests at significance level $\alpha=0.05$.
\end{tablenotes}
\end{threeparttable}
	\end{adjustbox}
\end{table}















==> tables/backtesting_sp500.tex <==
\begin{table}[ht]
	\centering
		\caption{S\&P 500 backtesting results}
		\vspace{-0.2cm}
	\label{tab:backtesting_sp500}
	\begin{adjustbox}{max width=0.8\textwidth}
	\begin{threeparttable}
\begin{tabular}{l  c ......}
\toprule
 &     \mc{LF var.} &          \mc{Mean} &         \mc{SD} &      \mc{AE} &     \mc{LR$_{uc}$} &       \mc{LR$_{cc}$} & \mc{DQ}\\
\midrule
\cellcolor{gray!50}MF--Q--ARCH--X & $\Delta IP_t$ & -1.055 & 0.562 & 0.938 & 0.654 & 0.901 & 0.698  \\ 
\cellcolor{gray!50}MF--Q--ARCH--X & $\Delta HS_t$ & -1.083 & 0.570 & 0.812 & 0.169 & 0.368 & 0.830  \\ 
 \cellcolor{gray!50}MF--Q--ARCH--X & $NAI_t$ & -1.071 & 0.583 & 0.938 & 0.654 & 0.901 & 0.989 \\ 
 \cellcolor{gray!50}MF--Q--ARCH & $\Delta IP_t$ & -1.085 & 0.433 & 0.917 & 0.548 & 0.663 & 0.735 \\ 
 \cellcolor{gray!50}MF--Q--ARCH & $\Delta HS_t$ & -1.121 & 0.434 & 0.958 & 0.766 & 0.493 & 0.473 \\ 
 \cellcolor{gray!50}MF--Q--ARCH & $NAI_t$ & -1.131 & 0.417 & 1.000 & 1.000 & 0.295 & 0.122 \\ 
  Q--ARCH &  & -1.104 & 0.426 & 0.938 & 0.654 & 0.426 & 0.738  \\
 SAV &  & -0.948 & 0.456 & 1.125 & 0.383 & 0.187 & 0.016 \\ 
 \cellcolor{gray!50}AS &  & -0.941 & 0.470 & 1.167 & 0.248 & 0.470 & 0.415  \\ 
  IG &  & -1.211 & 0.357 & 0.708 & 0.029 & 0.033 & 0.118  \\  
GARCH &  & -1.167 & 0.360 & 0.729 & 0.044 & 0.051 & 0.023 \\ 
  GARCH--t &  & -1.129 & 0.360 & 0.875 & 0.364 & 0.228 & 0.009  \\ 
   GJR &  & -1.188 & 0.434 & 0.729 & 0.044 & 0.051 & 0.195  \\ 
   \cellcolor{gray!50}GJR--t &  & -1.149 & 0.456 & 0.833 & 0.223 & 0.296 & 0.149 \\ 
  RiskMetrics &  & -1.186 & 0.414 & 0.750 & 0.063 & 0.078 & 0.108 \\ 
  GARCH--MIDAS & $\Delta IP_t$ & -1.238 & 0.543 & 0.688 & 0.019 & 0.047 & 0.046  \\ 
 GARCH--MIDAS & $\Delta HS_t$ & -1.242 & 0.480 & 0.729 & 0.044 & 0.051 & 0.171  \\ 
   GARCH--MIDAS & $NAI_t$ & -1.197 & 0.518 & 0.812 & 0.169 & 0.223 & 0.043  \\ 
\bottomrule
 \end{tabular}
	\begin{tablenotes}[flushleft]
   \setlength\labelsep{0pt}
   \linespread{1.25}
\item  \textbf{Notes}:  The table reports the backtesting results for the models in the first column, for the out-of-sample period, which starts on May 2, 2016 and ends on February 28, 2020 (960 days). The models with the \virg{--X} label include the realized volatility (see Eq. \eqref{eq:larch_midas_x}). Column \virg{LF var.} reports the low--frequency variables. Columns Mean and SD are the sample averages and standard deviations for the VaR measures. Column {AE} denotes the Actual over Expected exceedance ratio. Columns LR$_{uc}$ and LR$_{cc}$, report the p-values of the Unconditional and Conditional coverage tests. Finally, column DQ represents the p-value of the Dynamic Quantile test. Shades of gray denote that the model passes the LR$_{uc}$, LR$_{cc}$ and DQ tests at significance level $\alpha=0.05$.
\end{tablenotes}
\end{threeparttable}
	\end{adjustbox}
\end{table}

==> tables/in_sample_estimates.tex <==
\begin{table}[htbp]
%\tiny
\caption{Q--ARCH--MIDAS--X, Q--ARCH--MIDAS and Q--ARCH estimates. S\&P 500, $\tau=0.05$}
\label{tab:ARCH_est_sp500}       % Give a unique label
\vspace{-0.2cm}    
\resizebox{1\textwidth}{!}{%
\begin{tabular}{l ... ... .}
\toprule
  & \mc{Q--ARCH--MIDAS--X} & \mc{Q--ARCH--MIDAS--X} & \mc{Q--ARCH--MIDAS--X}& \mc{Q--ARCH--MIDAS} & \mc{Q--ARCH--MIDAS} & \mc{Q--ARCH--MIDAS}& \mc{Q--ARCH} \\
\midrule
$MV_t$& \mc{$\Delta IP_{t}$} & \mc{$\Delta HS_{t}$} & \mc{$NAI_{t}$} & \mc{$\Delta IP_{t}$}& \mc{$\Delta HS_{t}$} & \mc{$NAI_{t}$}\\
 \addlinespace
 \hdashline
 \addlinespace
$\beta_0(\tau)$ & -0.283^{***} & -0.306^{***} & -0.336^{***} & -0.404^{***} & -0.453^{***} & -0.477^{***} & -0.51^{***}  \\
              & (0.062)      & (0.065)      & (0.059)      & (0.073)      & (0.095)      & (0.073)      & (0.09)       \\
 $\beta_1(\tau)$ & 0.145^{***}  & 0.17^{***}   & 0.141^{***}  & -0.001^{}    & -0.019^{}    & 0.007^{}     & -0.037^{}    \\
              & (0.05)       & (0.049)      & (0.048)      & (0.054)      & (0.064)      & (0.056)      & (0.069)      \\
$\beta_2(\tau)$ & -0.09^{*}    & -0.104^{**}  & -0.124^{***} & -0.246^{***} & -0.318^{***} & -0.309^{***} & -0.311^{***} \\
               & (0.049)      & (0.047)      & (0.047)      & (0.054)      & (0.064)      & (0.056)      & (0.068)      \\
$\beta_3(\tau)$ & 0.012^{}     & 0.036^{}     & 0.029^{}     & -0.098^{*}   & -0.129^{**}  & -0.166^{***} & -0.136^{**}  \\
             & (0.047)      & (0.045)      & (0.045)      & (0.054)      & (0.064)      & (0.056)      & (0.069)      \\
$\beta_4(\tau)$ & -0.105^{**}  & -0.087^{**}  & -0.095^{**}  & -0.325^{***} & -0.306^{***} & -0.258^{***} & -0.372^{***} \\
             & (0.046)      & (0.044)      & (0.044)      & (0.054)      & (0.064)      & (0.055)      & (0.068)      \\
 $\beta_5(\tau)$ & -0.121^{***} & -0.112^{**}  & -0.082^{*}   & -0.178^{***} & -0.236^{***} & -0.153^{***} & -0.232^{***} \\
               & (0.045)      & (0.044)      & (0.043)      & (0.054)      & (0.064)      & (0.055)      & (0.068)      \\
 $\beta_6(\tau)$ & -0.152^{***} & -0.148^{***} & -0.167^{***} & -0.207^{***} & -0.208^{***} & -0.204^{***} & -0.225^{***} \\
                & (0.045)      & (0.044)      & (0.044)      & (0.054)      & (0.064)      & (0.056)      & (0.069)      \\
$\beta_7(\tau)$ & -0.105^{**}  & -0.119^{***} & -0.105^{**}  & -0.163^{***} & -0.138^{**}  & -0.129^{**}  & -0.121^{*}   \\
                & (0.045)      & (0.044)      & (0.044)      & (0.054)      & (0.064)      & (0.056)      & (0.068)      \\
 $\beta_8(\tau)$ & -0.122^{***} & -0.111^{**}  & -0.11^{**}   & -0.186^{***} & -0.187^{***} & -0.172^{***} & -0.189^{***} \\
                & (0.045)      & (0.044)      & (0.044)      & (0.054)      & (0.064)      & (0.056)      & (0.069)      \\
 $\beta_X(\tau)$ & -0.942^{***} & -1.079^{***} & -1.004^{***} &      &        &      &      \\
               & (0.103)      & (0.098)      & (0.098)      &        & &      &         \\
 $\theta(\tau)$   & -0.499^{***} & -0.044^{**}  & -0.143^{***} & -0.697^{***} & -0.095^{**}  & -0.374^{***} &       \\
               & (0.117)      & (0.022)      & (0.054)      & (0.126)      & (0.043)      & (0.068)      &      \\

\bottomrule
\addlinespace
\end{tabular}
}
{\footnotesize 
\textbf{Notes}: The table reports the estimates at $\tau$ level for the Q--ARCH models. Number in parentheses are the standard errors, computed considering the estimate of the asymptotic covariance matrix as discussed in \cite{Koenker:Bassett:1978}.
$^{*}$, $^{**}$ and $^{***}$ represent the significance at levels $10\%, 5\%, 1\%$, respectively. The row $(MV_t)$ indicates the MIDAS variable for each model. The models with the \virg{--X} label include the realized volatility (see Eq. \eqref{eq:larch_midas_x}). Sample period: January 2001 to April 2016 (3846 obs.).
}
\end{table}


\begin{table}[htbp]
%\tiny
\caption{Q--ARCH--MIDAS--X, Q--ARCH--MIDAS and Q--ARCH estimates. NASDAQ, $\tau=0.05$}
\label{tab:ARCH_est_nas}       % Give a unique label
\vspace{-0.2cm}    
\resizebox{1\textwidth}{!}{%
\begin{tabular}{l ... ... .}
\toprule
  & \mc{Q--ARCH--MIDAS--X} & \mc{Q--ARCH--MIDAS--X} & \mc{Q--ARCH--MIDAS--X}& \mc{Q--ARCH--MIDAS} & \mc{Q--ARCH--MIDAS} & \mc{Q--ARCH--MIDAS}& \mc{Q--ARCH} \\
\midrule
$MV_t$& \mc{$\Delta IP_{t}$} & \mc{$\Delta HS_{t}$} & \mc{$NAI_{t}$} & \mc{$\Delta IP_{t}$}& \mc{$\Delta HS_{t}$} & \mc{$NAI_{t}$}\\
 \addlinespace
 \hdashline
 \addlinespace
$\beta_0(\tau)$ & -0.4^{***}   & -0.345^{***} & -0.39^{***}  & -0.579^{***} & -0.556^{***} & -0.666^{***} & -0.62^{***}  \\
                & (0.057)      & (0.071)      & (0.071)      & (0.085)      & (0.115)      & (0.077)      & (0.088)      \\
  $\beta_1(\tau)$ & 0.174^{***}  & 0.174^{***}  & 0.199^{***}  & 0.007^{}     & 0.033^{}     & 0.044^{}     & -0.01^{}     \\
                & (0.039)      & (0.044)      & (0.049)      & (0.054)      & (0.066)      & (0.051)      & (0.058)      \\
 $\beta_2(\tau)$ & -0.077^{**}  & -0.096^{**}  & -0.086^{*}   & -0.289^{***} & -0.269^{***} & -0.276^{***} & -0.267^{***} \\
                & (0.038)      & (0.044)      & (0.049)      & (0.054)      & (0.066)      & (0.051)      & (0.058)      \\
 $\beta_3(\tau)$ & -0.087^{**}  & -0.084^{**}  & -0.073^{}    & -0.224^{***} & -0.275^{***} & -0.233^{***} & -0.267^{***} \\
                & (0.036)      & (0.041)      & (0.046)      & (0.055)      & (0.066)      & (0.051)      & (0.058)      \\
 $\beta_4(\tau)$ & -0.133^{***} & -0.143^{***} & -0.158^{***} & -0.279^{***} & -0.296^{***} & -0.238^{***} & -0.272^{***} \\
                & (0.035)      & (0.041)      & (0.045)      & (0.055)      & (0.066)      & (0.051)      & (0.058)      \\
 $\beta_5(\tau)$ & -0.1^{***}   & -0.136^{***} & -0.129^{***} & -0.122^{**}  & -0.166^{**}  & -0.143^{***} & -0.174^{***} \\
                & (0.035)      & (0.04)       & (0.044)      & (0.055)      & (0.066)      & (0.051)      & (0.058)      \\
 $\beta_6(\tau)$ & -0.076^{**}  & -0.119^{***} & -0.111^{**}  & -0.241^{***} & -0.242^{***} & -0.211^{***} & -0.219^{***} \\
                & (0.035)      & (0.04)       & (0.045)      & (0.054)      & (0.066)      & (0.051)      & (0.058)      \\
$\beta_7(\tau)$ & -0.038^{}    & -0.026^{}    & -0.024^{}    & -0.149^{***} & -0.154^{**}  & -0.111^{**}  & -0.205^{***} \\
                & (0.035)      & (0.04)       & (0.044)      & (0.054)      & (0.066)      & (0.051)      & (0.058)      \\
 $\beta_8(\tau)$ & -0.055^{}    & -0.046^{}    & -0.044^{}    & -0.122^{**}  & -0.139^{**}  & -0.145^{***} & -0.135^{**}  \\
                & (0.035)      & (0.04)       & (0.044)      & (0.054)      & (0.066)      & (0.051)      & (0.058)      \\
 $\beta_X(\tau)$ & -1.145^{***} & -1.206^{***} & -1.21^{***}  &        &        &       &        \\
                & (0.095)      & (0.107)      & (0.121)      &        &        & &        \\
 $\theta(\tau)$   & -0.259^{***} & -0.022^{}    & -0.08^{}     & -0.39^{***}  & -0.056^{}    & -0.332^{***} &        \\
                & (0.083)      & (0.022)      & (0.058)      & (0.13)       & (0.039)      & (0.066)      &       \\
\bottomrule
\addlinespace
\end{tabular}
}
{\footnotesize 
\textbf{Notes}: The table reports the estimates at $\tau$ level for the Q--ARCH models. Number in parentheses are the standard errors, computed considering the estimate of the asymptotic covariance matrix as discussed in \cite{Koenker:Bassett:1978}.
$^{*}$, $^{**}$ and $^{***}$ represent the significance at levels $10\%, 5\%, 1\%$, respectively. The row $(MV_t)$ indicates the MIDAS variable for each model. The models with the \virg{--X} label include the realized volatility (see Eq. \eqref{eq:larch_midas_x}).  Sample period: January 2001 to April 2016 (3845 obs.).
}
\end{table}



\begin{table}[htbp]
%\tiny
\caption{Q--ARCH--MIDAS--X, Q--ARCH--MIDAS and Q--ARCH estimates. Dow Jones, $\tau=0.05$}
\label{tab:ARCH_est_dow}       % Give a unique label
\vspace{-0.2cm}    
\resizebox{1\textwidth}{!}{%
\begin{tabular}{l ... ... .}
\toprule
  & \mc{Q--ARCH--MIDAS--X} & \mc{Q--ARCH--MIDAS--X} & \mc{Q--ARCH--MIDAS--X}& \mc{Q--ARCH--MIDAS} & \mc{Q--ARCH--MIDAS} & \mc{Q--ARCH--MIDAS}& \mc{Q--ARCH} \\
\midrule
$MV_t$& \mc{$\Delta IP_{t}$} & \mc{$\Delta HS_{t}$} & \mc{$NAI_{t}$} & \mc{$\Delta IP_{t}$}& \mc{$\Delta HS_{t}$} & \mc{$NAI_{t}$}\\
 \addlinespace
 \hdashline
 \addlinespace
$\beta_0(\tau)$ & -0.319^{***} & -0.346^{***} & -0.401^{***} & -0.42^{***}  & -0.359^{***} & -0.457^{***} & -0.447^{***} \\
                & (0.083)      & (0.08)       & (0.074)      & (0.066)      & (0.066)      & (0.061)      & (0.074)      \\
  $\beta_1(\tau)$ & 0.096^{}     & 0.101^{*}    & 0.078^{}     & -0.083^{*}   & -0.126^{***} & -0.117^{**}  & -0.115^{**}  \\
                 & (0.069)      & (0.061)      & (0.063)      & (0.05)       & (0.046)      & (0.047)      & (0.057)      \\
  $\beta_2(\tau)$ & -0.159^{**}  & -0.127^{**}  & -0.155^{***} & -0.286^{***} & -0.349^{***} & -0.364^{***} & -0.357^{***} \\
                & (0.064)      & (0.056)      & (0.059)      & (0.049)      & (0.046)      & (0.047)      & (0.057)      \\
  $\beta_3(\tau)$ & -0.022^{}    & 0.002^{}     & -0.051^{}    & -0.156^{***} & -0.168^{***} & -0.092^{**}  & -0.146^{**}  \\
                 & (0.063)      & (0.055)      & (0.058)      & (0.05)       & (0.046)      & (0.047)      & (0.057)      \\
  $\beta_4(\tau)$ & -0.105^{*}   & -0.078^{}    & -0.088^{}    & -0.218^{***} & -0.252^{***} & -0.167^{***} & -0.245^{***} \\
                & (0.062)      & (0.054)      & (0.056)      & (0.049)      & (0.045)      & (0.046)      & (0.057)      \\
 $\beta_5(\tau)$ & -0.096^{}    & -0.116^{**}  & -0.138^{**}  & -0.178^{***} & -0.153^{***} & -0.184^{***} & -0.207^{***} \\
                & (0.061)      & (0.054)      & (0.056)      & (0.049)      & (0.045)      & (0.046)      & (0.057)      \\
$\beta_6(\tau)$ & -0.127^{**}  & -0.131^{**}  & -0.144^{***} & -0.165^{***} & -0.173^{***} & -0.15^{***}  & -0.192^{***} \\
               & (0.061)      & (0.054)      & (0.056)      & (0.049)      & (0.046)      & (0.047)      & (0.057)      \\
 $\beta_7(\tau)$ & -0.092^{}    & -0.112^{**}  & -0.096^{*}   & -0.148^{***} & -0.206^{***} & -0.149^{***} & -0.15^{***}  \\
                & (0.061)      & (0.054)      & (0.056)      & (0.049)      & (0.046)      & (0.047)      & (0.057)      \\
$\beta_8(\tau)$ & -0.157^{***} & -0.123^{**}  & -0.134^{**}  & -0.171^{***} & -0.223^{***} & -0.176^{***} & -0.25^{***}  \\
               & (0.061)      & (0.053)      & (0.056)      & (0.049)      & (0.046)      & (0.047)      & (0.057)      \\
$\beta_X(\tau)$ & -0.738^{***} & -0.873^{***} & -0.645^{***} &       &        & &        \\
                & (0.129)      & (0.113)      & (0.118)      &         & &       &        \\
$\theta(\tau)$   & -0.587^{***} & -0.065^{*}   & -0.278^{***} & -0.546^{***} & -0.058^{**}  & -0.334^{***} &       \\
              & (0.167)      & (0.034)      & (0.068)      & (0.117)      & (0.025)      & (0.057)      &        \\

\bottomrule
\addlinespace
\end{tabular}
}
{\footnotesize 
\textbf{Notes}: The table reports the estimates at $\tau$ level for the Q--ARCH models. Number in parentheses are the standard errors, computed considering the estimate of the asymptotic covariance matrix as discussed in \cite{Koenker:Bassett:1978}.
$^{*}$, $^{**}$ and $^{***}$ represent the significance at levels $10\%, 5\%, 1\%$, respectively. The row $(MV_t)$ indicates the MIDAS variable for each model. The models with the \virg{--X} label include the realized volatility (see Eq. \eqref{eq:larch_midas_x}).  Sample period: January 2001 to April 2016 (3846 obs.).
}
\end{table}

==> tables/mcs.tex <==
\begin{table}[ht]
	\centering
		\caption{Superior set of models provided by the MCS procedure for each index 	\label{tab:mcs}}
\vspace{-0.2cm}   
\centering 
\begin{adjustbox}{max width=0.8\textwidth}	\begin{threeparttable}
\begin{tabular}{l  c .. .. ..}
\toprule
& & \multicolumn{2}{c}{S\&P 500}& \multicolumn{2}{c}{NASDAQ} & \multicolumn{2}{c}{Dow Jones}\\
\midrule
 &     \mc{LF var.} &          \mc{$\overline{\ell}$} &    \mc{SSM}      &         \mc{$\overline{\ell}$} &    \mc{SSM}&  \mc{$\overline{\ell}$}&    \mc{SSM}  \\
 \addlinespace
 \hdashline
 \addlinespace
MF--Q--ARCH--X 	&	 $\Delta IP_t$ 	&	7.985	&	\mc{\textcolor{black}{\circled{\scriptsize 25}, }\circled{\scriptsize 10}}	&	9.479	&	\mc{\textcolor{black}{\circled{\scriptsize 25}, }\circled{\scriptsize 10}}	&	7.942	&	\mc{\textcolor{black}{\circled{\scriptsize 25}, }\circled{\scriptsize 10}}	\\
MF--Q--ARCH--X 	&	 $\Delta HS_t$ 	&	7.907	&	\mc{\textcolor{black}{\circled{\scriptsize 25}, }\circled{\scriptsize 10}}	&	9.592	&	\mc{\textcolor{black}{\circled{\scriptsize 25}, }\circled{\scriptsize 10}}	&	7.967	&	\mc{\textcolor{black}{\circled{\scriptsize 25}, }\circled{\scriptsize 10}}	\\
 MF--Q--ARCH--X 	&	 $NAI_t$ 	&	7.997	&	\mc{\textcolor{black}{\circled{\scriptsize 25}, }\circled{\scriptsize 10}}	&	9.579	&	\mc{\textcolor{black}{\circled{\scriptsize 25}, }\circled{\scriptsize 10}}	&	8.023	&	\mc{\textcolor{black}{\circled{\scriptsize 25}, }\circled{\scriptsize 10}}	\\
 MF--Q--ARCH 	&	 $\Delta IP_t$ 	&	8.412	&		&	10.291	&		&	8.594	&		\\
 MF--Q--ARCH 	&	 $\Delta HS_t$ 	&	8.578	&		&	10.442	&		&	8.603	&		\\
 MF--Q--ARCH 	&	 $NAI_t$ 	&	8.626	&		&	10.419	&		&	8.673	&		\\
  Q--ARCH 	&	  	&	8.425	&		&	10.408	&		&	8.583	&		\\
  SAV 	&	  	&	8.167	&	\mc{\textcolor{black}{\circled{\scriptsize 25}, }\circled{\scriptsize 10}}	&	10.488	&		&	8.279	&	\mc{\textcolor{white}{\circled{\scriptsize 25}, }\circled{\scriptsize 10}}	\\
 AS 	&	  	&	8.124	&	\mc{\textcolor{black}{\circled{\scriptsize 25}, }\circled{\scriptsize 10}}	&	10.399	&		&	8.248	&	\mc{\textcolor{white}{\circled{\scriptsize 25}, }\circled{\scriptsize 10}}	\\
  IG 	&	  	&	8.640	&		&	10.505	&		&	8.872	&		\\
GARCH 	&	  	&	8.527	&		&	10.376	&		&	8.841	&		\\
  GARCH--t 	&	  	&	8.494	&		&	10.420	&		&	8.824	&		\\
   GJR 	&	  	&	8.535	&		&	10.348	&		&	8.785	&		\\
   GJR--t 	&	  	&	8.459	&	\mc{\textcolor{white}{\circled{\scriptsize 25}, }\circled{\scriptsize 10}}	&	10.386	&		&	8.736	&		\\
  RiskMetrics 	&	  	&	8.464	&	\mc{\textcolor{white}{\circled{\scriptsize 25}, }\circled{\scriptsize 10}}	&	10.348	&		&	8.786	&		\\
  GARCH--MIDAS 	&	 $\Delta IP_t$ 	&	8.769	&		&	10.438	&		&	9.099	&		\\
 GARCH--MIDAS 	&	 $\Delta HS_t$ 	&	8.757	&		&	10.341	&		&	8.924	&		\\
  GARCH--MIDAS 	&	 $NAI_t$ 	&	8.658	&		&	10.461	&		&	9.081	&		\\
\bottomrule
\addlinespace
 \end{tabular}
 \vspace{-0.2cm}
	\begin{tablenotes}[flushleft]
   \setlength\labelsep{0pt}
   \linespread{1.25}
\item  \textbf{Notes}: The table reports the inclusion in the SSM according to the MCS procedure. Column \virg{LF var.} reports the low--frequency variables. Column $\overline{\ell}$  represents the averages of the loss function in \eqref{eq:loss_funct}, used in the MCS procedure. The out-of-sample period, which starts on May 2, 2016 and ends on February 28, 2020 (960, 959 e 958 days, respectively, for S\&P 500, NASDAQ and Dow Jones). The models with the \virg{--X} label include the realized volatility (see Eq. \eqref{eq:larch_midas_x}).  Symbols  \circled{\scriptsize 25} and \circled{\scriptsize 10} denote inclusion in the SSM at significance level $\alpha=0.25$ and $\alpha=0.10$, respectively. 
\end{tablenotes}
\end{threeparttable}
\end{adjustbox}
\end{table}
